Improved Path-length Regret Bounds for Bandits

We study adaptive regret bounds in terms of the variation of the losses (the so-called path-length bounds) for both multi-armed bandit and more generally linear bandit. We first show that the seemingly suboptimal path-length bound of (Wei and Luo, 2018) is in fact not improvable for adaptive adversary. Despite this negative result, we then develop two new algorithms, one that strictly improves over (Wei and Luo, 2018) with a smaller path-length measure, and the other which improves over (Wei and Luo, 2018) for oblivious adversary when the path-length is large. Our algorithms are based on the well-studied optimistic mirror descent framework, but importantly with several novel techniques, including new optimistic predictions, a slight bias towards recently selected arms, and the use of a hybrid regularizer similar to that of (Bubeck et al., 2018). Furthermore, we extend our results to linear bandit by showing a reduction to obtaining dynamic regret for a full-information problem, followed by a further reduction to convex body chasing. We propose a simple greedy chasing algorithm for squared 2-norm, leading to new dynamic regret results and as a consequence the first path-length regret for general linear bandit as well.

==> linear_bandit_old_version.tex <==
\subsection{A detour via convex body chasing}
We first describe the general convex body chasing problem
(overloading some of our notations for convenience).
For each time $t=1, \ldots, T$,
the algorithm is presented with a convex set $\calK_t$ in the metric space and then needs to select a point $m_t \in \calK_t$.
The algorithm performance is measured by the total movement cost 
$\sum_{t=1}^{T-1} \dist(m_t, m_{t+1})$ where $\dist(\cdot, \cdot)$ is some distance function (usually a metric).
The algorithm is said to be $\omega$-competitive if its total movement cost is at most $\omega\sum_{t=1}^{T-1} \dist(m_t^\star, m_{t+1}^\star)$ for any sequence $m_1^\star \in \calK_1, \ldots, m_T^\star \in \calK_T$.

Our problem of finding the optimistic prediction sequence can be seen as an instance of convex body chasing by defining $\calK_{t} \triangleq \{m \in \calB: \inner{w_{t-1}, m} = c_{t-1}\}$ for $t \geq 2$ (and $\calK_{1} = \calB$)
and using the squared 2-norm as the distance function.
Indeed, suppose $m_t \in \calK_{t}$ for all $t$, 
then we can bound the last term of \pref{eqn:SCRiBLe} as follows:
\[
\sum_{t=1}^{T-1} \inn{w_t, \ell_t - m_t}^2 
= \sum_{t=1}^{T-1} \inn{w_t, m_{t+1} - m_t}^2 
\leq \sum_{t=1}^{T-1} \norm{m_{t+1} - m_t}^2,
\]
which is exactly the total movement cost of the sequence $m_1, \ldots, m_T$.
Therefore, if the sequence is competitive,
then we can further bound the above by some factor of the movement cost of any sequence $m_1^\star \in \calK_1, \ldots, m_T^\star \in \calK_T$,
and in particular, the sequence $\ell_1, \ldots, \ell_T$, 
which then leads to a path-length regret bound in terms of $\sum_{t=1}^{T-1} \norm{\ell_{t+1} - \ell_t}^2$.

Unfortunately, no existing convex body chasing algorithms can solve our problem:
first, existing works all focus on metric space and squared 2-norm is not a metric;
second, even if we bound $\norm{m_{t+1} - m_t}^2$ by $2\norm{m_{t+1} - m_t}$ so the problem fits into the typical setting studied in the literature,
the best known result is a $2^{\order(d)}$-competitive algorithm~\citep{bubeck2018competitively},
\HLcomment{is this correct?}
leading to a regret bound that is exponential in the dimension $d$.

However, we show that a very natural greedy approach is ``competitive'' in a slightly weaker sense where we measure the movement cost of the algorithm by squared 2-norm and the movement cost of the benchmark by 2-norm.
The greedy approach is simply to project $m_t$ onto $\calK_{t+1}$ as the next point $m_{t+1}$ (\pref{line:chasing} of \pref{alg:linear_bandit}):
\[
m_{t+1} = \proj_{\calK_{t+1}}(m_t) \triangleq \argmin_{m \in \calK_{t+1}}\norm{m - m_t}.
\]
We prove the following result of this greedy approach.

\begin{lemma}\label{lem:chasing}
\pref{line:chasing} of \pref{alg:linear_bandit} ensures for any sequence $m_1^\star \in \calK_1, \ldots, m_{T+1}^\star \in \calK_{T+1}$, 
\[
\sum_{t=1}^{T} \inn{w_t, \ell_t - m_t}^2 
\leq 1 + 6\sum_{t=1}^{T} \norm{m_t^\star - m_{t+1}^\star}.
\]
\end{lemma}
\begin{proof}
Since $m_{t+1}$ is the projection of $m_{t}$ on $\calK_{t+1}$ and also $m_{t+1}^\star \in \calK_{t+1}$,
by the generalized Pythagorean theorem we have
\[
\norm{m_{t+1}-m_{t+1}^\star}^2 + \norm{m_{t+1}-m_{t}}^2 \leq \norm{m_{t} - m_{t+1}^\star}^2.
\]
On the other hand, by triangle inequality we also have
\begin{align*}
\norm{m_{t} - m_{t+1}^\star}^2
&\leq \left(\norm{m_{t} - m_{t}^\star} + \norm{m_{t}^\star - m_{t+1}^\star}\right)^2 \\
&= \norm{m_{t} - m_{t}^\star}^2 + 2 \norm{m_{t} - m_{t}^\star}\norm{m_{t}^\star - m_{t+1}^\star} + \norm{m_{t}^\star - m_{t+1}^\star}^2 \\
&\leq \norm{m_{t} - m_{t}^\star}^2 + 6\norm{m_{t}^\star - m_{t+1}^\star}.
\end{align*}
Combining the two inequalities above, summing over $t$, and telescoping give
\[
\sum_{t=1}^T \norm{m_{t+1}-m_{t}}^2
\leq \norm{m_{1} - m_{1}^\star}^2 %- \norm{m_{T+1} - m_{T+1}^\star}^2  
+ 6\sum_{t=1}^T \norm{m_{t}^\star - m_{t+1}^\star}
\leq 1 + 6\sum_{t=1}^T \norm{m_{t}^\star - m_{t+1}^\star}.
\]
Finally realizing $\inn{w_t, \ell_t - m_t}^2 = \inn{w_t, m_{t+1} - m_t}^2 \leq \norm{m_{t+1}-m_{t}}^2$ finishes the proof.
\end{proof}

The final regret bound of \pref{alg:linear_bandit} shown in the following theorem is then a direct combination of \pref{eqn:SCRiBLe}, \pref{lem:chasing}, and the fact $\ell_t \in \calK_{t+1}$.

\begin{theorem}\label{thm:linear_bandit}
\pref{alg:linear_bandit} ensures
\[
\reg = \order\left(\frac{\nu\ln T}{\eta} + \eta d^2 \E\left[\sum_{t=1}^T \norm{\ell_{t} - \ell_{t-1}}\right]\right),
\]
which is of order $\otil\left( d\sqrt{\nu V_2} \right)$ with the optimal $\eta$.
\end{theorem}

It is well known that any convex body in $d$ dimension admits an $\order(d)$-self-concordant barrier,
and therefore \pref{alg:linear_bandit} admits a regret bound $\otil\left( d^{3/2}\sqrt{V_2} \right)$.
Note that the construction of the classic $\Omega(d\sqrt{T})$ lower bound for linear bandit~\citep{dani2008price} also directly implies a lower bound of $\Omega(d\sqrt{V_2})$.
The suboptimal dependence on $d$ in our bound inherits directly from the suboptimality of SCRiBLe,
and we expect that using the entropic barrier instead as discussed in~\citep{bubeck2015entropic} improves the dependence to $\order(d)$  
(details are omitted and left as a future direction).

\subsection{A different view via dynamic regret}
In this subsection we briefly discuss a different view of the problem of selecting the optimistic prediction sequence and why existing works do not provide satisfactory solutions.
\citet{rakhlin2013online} suggest treating this as another online learning problem over some fixed set of predictable processes and propose strategies to learn the best predictable process.
As a simple example, consider the following online learning formulation:
at each time $t$ the algorithm selects $m_t \in \calB$ and then observes the loss function $f_t(m) = \inn{w_t, \ell_t - m}^2 = (c_t - \inn{w_t, m})^2$ which is exp-concave.
Note that this is a full information problem even though $\ell_t$ is unknown
and is in fact the standard problem of online linear regression with squared loss.
Applying Online Newton Step~\citep{hazan2007logarithmic} to learn $m_t$ then ensures
\begin{align*}
&\sum_{t=1}^T \inn{w_t, \ell_t - m_t}^2
\leq \min_{m^\star\in \calB} \sum_{t=1}^T \inn{w_t, \ell_t - m^\star}^2 + \order(d\ln T) \\
&\leq \min_{m^\star\in \calB} \sum_{t=1}^T \norm{\ell_t - m^\star}^2 + \order(d\ln T)
\leq \sum_{t=1}^T \norm{\ell_t - \frac{1}{T}\sum_{s=1}^T\ell_s}^2 + \order(d\ln T).
\end{align*}
Combining the above with \pref{eqn:SCRiBLe} then recovers the main result of~\citep{hazan2011better} with a different approach.
(This observation was not made in~\citep{rakhlin2013online} though.)

However, competing with a fixed $m^\star$ is not adequate for getting path-length bound.
Instead in this case we need to have a {\it dynamic regret} bound~\citep{zinkevich2003online} that allows the algorithm to compete with any sequence $m_1^\star, \ldots, m_T^\star$ instead of a fixed $m^\star$, and typically such bound depends on either the variation of the loss functions or the competitor sequence.
For example, recent results of~\citep{zhang2018adaptive} imply a strategy to ensure for any $m_1^\star, \ldots, m_T^\star\in \calB$
\begin{align*}
&\sum_{t=1}^T \inn{w_t, \ell_t - m_t}^2
\leq \sum_{t=1}^T \inn{w_t, \ell_t - m_t^\star}^2 + \order\left(\sqrt{T\sum_{t=2}^T \norm{m_t^\star-m_{t-1}^\star}}\right),
\end{align*}
which then implies $\sum_{t=1}^T \inn{w_t, \ell_t - m_t}^2 \leq \order(\sqrt{TV_2})$ by picking $m_t^\star = \ell_t$.
Combining with \pref{eqn:SCRiBLe} then leads to a regret bound $\otil(d\sqrt{\nu}(TV_2)^{1/4})$, worse than our bound in \pref{thm:linear_bandit}.
Several works~\citep{jadbabaie2015online, mokhtari2016online, Yang2016tracking, zhang2017improved} propose improved dynamic regret bounds, but all under extra conditions that do not hold for our problem.
Our greedy approach and \pref{lem:chasing} can thus be seen as a new and improved result on dynamic regret for online linear regression.

%========Previous proof==========
%Using optimistic SCRiBLe algorithm for linear bandit, one can achieve the following expected regret bound: 
%\HLcomment{use entropic barrier to reduce $d^2$ to $d$?}
%\begin{align*}
%\E[\reg_T] = \mathcal{O}\left(\frac{d\ln T}{\eta} + d^2\E\left[ \sum_{t=1}^T \inner{\tilde{w}_t, \ell_t-m_t}^2\right]  \right). 
%\end{align*}
%Below is a proposal of setting $m_t$ for obtaining a path-length bound: 
%\begin{align*}
%m_{t+1}' &= \Pi_t(m_t), \\
%m_{t+1} &= \Pi(m_{t+1}'), 
%\end{align*}
%where $m_1 = \mathbf{0}$, $\Pi_t(\cdot)$ is the $\ell_2$-projection operator onto the $(d-1)$-dimension plane 
%$S_t=\{x\in \mathbb{R}^d : \tilde{w}_t^\top x - \tilde{w}_t^\top \ell_t=0\}$,
%and $\Pi(\cdot)$ is the $\ell_2$-projection operator onto the set where $\ell_t$'s are from
%(or just a superset such as $\{m \in \fR^d: \norm{m}_2 \leq G\}$ if $\norm{\ell_t}_2 \leq G$).
%
%This is actually a generalization of the MAB algorithm of \citet{wei2018more}. Recall in that case $m_{t+1,i}=\ell_{\alpha_{t+1}(i),i}$. Below is an two-arm example where we assume the learner picks $2,2,1,2$ arms respectively in the first four rounds. 
%
%\begin{center}
%\includegraphics[width=8cm]{fig1}
%\end{center}
%
%In the above figure, one can see that $m_{t+1}$ is always a projection of $m_t$ onto $S_t$. And note that $m_1=(0,0), m_2=(0,\ell_{1,2}), m_3=(0,\ell_{2,2}), m_4=(\ell_{3,1},\ell_{2,2}), m_5=(\ell_{3,1}, \ell_{4,2})$, exactly following the formula $m_{t+1,i}=\ell_{\alpha_{t+1}(i),i}$. 
%Below is a picture to illustrate a more general case (assuming the projection $\Pi$ does nothing for simplicity).
%
%\begin{center}
%\includegraphics[width=8cm]{fig2}
%\end{center}
%
%%\begin{center}
%%\includegraphics[width=8cm]{fig3}
%%\end{center}
%
%\begin{theorem}
%Suppose $\norm{\tilde{w}_t}_2 \leq D$ and $\norm{\ell_t}_2 \leq G$ for all $t \in [T]$. The above scheme ensures:
%\[
%\sum_{t=1}^T \inner{\tilde{w}_t, \ell_t-m_t}^2 \leq 8GD^2(1+\ln T)\sum_{t=1}^T \norm{\ell_t - \ell_{t-1}}_2.
%\]
%\end{theorem}
%
%\begin{proof}
%Assume $\tilde{w}_t\neq \mathbf{0}$ and define $u_t=\frac{\tilde{w}_t}{\norm{\tilde{w}_t}}$. 
%Note that the update rule $m_{t+1}'=\Pi_t (m_t) $ can be written as 
%\begin{align}
%m_{t+1}' = m_t + u_t u_t^\top(\ell_t-m_t).  \label{eqn:update}
%\end{align}
%Thus we have
%\begin{gather}
%\ell_t-m_{t+1}' = (I-u_tu_t^\top)(\ell_t-m_t) = (I-u_tu_t^\top)(\ell_t-\ell_{t-1}) + (I-u_tu_t^\top)(\ell_{t-1}-m_t). \label{eqn:iteration}
%%m_{t+1}-m_t = u_tu_t^\top (\ell_t-m_t) = u_tu_t^\top (\ell_t-\ell_{t-1}) + u_tu_t^\top (\ell_{t-1}-m_t). 
%\end{gather}
%Define 
%\[
%\cos\phi_t= \frac{\norm{(I-u_tu_t^\top)(\ell_t-\ell_{t-1})}}{\norm{\ell_t-\ell_{t-1}}} \text{\quad and \quad} 
%\cos\theta_t= \frac{\norm{(I-u_tu_t^\top)(\ell_{t-1}-m_t)}}{\norm{\ell_{t-1}-m_t}}.
%\]
%Then by the second projection step of the algorithm and \pref{eqn:update} and~\pref{eqn:iteration}, we have
%\begin{align*}
%    \norm{\ell_t-m_{t+1}}&\leq\norm{\ell_t-m_{t+1}'}\leq \norm{(I-u_tu_t^\top)(\ell_t-\ell_{t-1})} + \norm{(I-u_tu_t^\top)(\ell_{t-1}-m_t)} \\
%    &=\norm{\ell_t-\ell_{t-1}}\cos\phi_t + \norm{\ell_{t-1}-m_t}\cos\theta_t, 
%\end{align*}
%and 
%\begin{align*}
%    \norm{m_{t}-m_{t+1}'} &=\norm{u_tu_t^\top(\ell_t-m_t)} \leq 
%    \norm{u_tu_t^\top(\ell_t-\ell_{t-1})} + \norm{u_tu_t^\top (\ell_{t-1}-m_t)}\\
%    &=\norm{\ell_t-\ell_{t-1}}\sin\phi_t + \norm{\ell_{t-1}-m_t}\sin\theta_t. 
%\end{align*}
%%
%Combining the above two inequalities, we get
%\begin{align*}
%    &\norm{m_t-m_{t+1}'}^2  \\
%    &\leq 2\norm{\ell_t-\ell_{t-1}}^2\sin^2\phi_t + 2\norm{\ell_{t-1}-m_t}^2\sin^2\theta_t \\
%    &\leq 4G\norm{\ell_t-\ell_{t-1}}\sin^2\phi_t + 4G\norm{\ell_{t-1}-m_t}\sin^2\theta_t \\
%    &\leq 4G\norm{\ell_t-\ell_{t-1}}\sin^2\phi_t + 4G\norm{\ell_{t-1}-\ell_{t-2}}\sin^2\theta_t\cos\phi_{t-1}+4G\norm{\ell_{t-2}-m_{t-1}}\sin^2\theta_t\cos\theta_{t-1} \\
%    &\leq 4G\norm{\ell_t-\ell_{t-1}}\sin^2\phi_t + 4G\norm{\ell_{t-1}-\ell_{t-2}}\sin^2\theta_t\cos\phi_{t-1}\\
%    & \ \ \ \ \ \ +4G\norm{\ell_{t-2}-\ell_{t-3}}\sin^2\theta_t\cos\theta_{t-1}\cos\phi_{t-2} + 4G\norm{\ell_{t-3}-m_{t-2}}\sin^2\theta_t\cos\theta_{t-1}\cos\theta_{t-2} \\
%    &\leq \cdots
%\end{align*}
%%
%So one can see that 
%\begin{align*}
%    \sum_{t=1}^T \inner{\tilde{w}_t, \ell_t-m_t}^2 = \sum_{t=1}^T \inner{\tilde{w}_t, m_{t+1}'-m_t}^2
%    \leq D^2\sum_{t=1}^T \norm{m_{t+1}'-m_t}^2 \leq 4GD^2\sum_{t=1}^T a_t \norm{\ell_t-\ell_{t-1}}, 
%\end{align*}
%where 
%\begin{align*}
%    a_t=\sin^2\phi_t + \sin^2\theta_{t+1}\cos\phi_t + \sin^2\theta_{t+2}\cos\theta_{t+1}\cos\phi_t + \sin^2\theta_{t+3}\cos\theta_{t+2}\cos\theta_{t+1}\cos\phi_t+\cdots.
%\end{align*}
%
%It remains to bound $a_t$. Fix $t$, and define $b_s=\sin^2\theta_s \cos\theta_{s-1}\cdots \cos\theta_{t+1}\cos\phi_t$ for $s > t$ and
%$b_t = \sin^2\phi_t$. Thus $a_t=\sum_{s=t}^T b_s$. By the fact $\cos\theta = \sqrt{1-\sin^2\theta}\leq 1-\frac{\sin^2\theta}{2}$, we have the following property: for $s > t$,
%\begin{align*}
%    b_s&=\sin^2\theta_s \cos\theta_{s-1}\cdots \cos\theta_{t+1}\cos\phi_t \\
%    &\leq \sin^2\theta_s \left(1-\frac{\sin^2\theta_{s-1}}{2}\right)\cdots\left(  1-\frac{\sin^2\theta_{t+1}}{2} \right)\left(1-  \frac{\sin^2\phi_{t}}{2} \right) \\
%    &\leq \left(1-\frac{b_{s-1}}{2}\right)\cdots \left(1-\frac{b_{t+1}}{2}\right)\left(1-\frac{b_{t}}{2}\right)
%    \leq \exp\left(-\frac{1}{2}\sum_{\tau = t}^{s-1}b_\tau \right). 
%\end{align*}
%Let $s^*$ be such that $\sum_{\tau = t}^{s^*-1}b_\tau\leq 2\ln T$ and 
%$\sum_{\tau = t}^{s^*}b_\tau > 2\ln T$ (if it does not exist, then clearly $a_t = \sum_{s=t}^T b_s \leq 2\ln T$). 
%We therefore have for all $s > s^*$, 
%$b_s \leq \exp\left(-\frac{1}{2}\sum_{\tau = t}^{s-1}b_\tau \right) \leq \exp\left(-\frac{1}{2}\sum_{\tau = t}^{s^*}b_\tau \right) = \frac{1}{T}$,
%and thus
%\[
%a_t = \sum_{\tau = t}^{s^*-1}b_\tau + b_{s^*} + \sum_{\tau = s^* + 1}^{T}b_\tau
%\leq 2\ln T + 1 + \sum_{\tau = s^* + 1}^{T}\frac{1}{T} \leq 2(1 + \ln T).
%\]
%\end{proof}
%========Previous proof==========

